Renormalisation of Quantum Cellular Automata

We study a coarse-graining procedure for quantum cellular automata on hypercubic lattices that consists in grouping neighboring cells into tiles and selecting a subspace within each tile. This is done in such a way that multiple evolution steps applied to this subspace can be viewed as a single evolution step of a new quantum cellular automaton, whose cells are the subspaces themselves. We derive a necessary and sufficient condition for renormalizability and use it to investigate the renormalization flow of cellular automata on a line, where the cells are qubits and the tiles are composed of two neighboring cells. The problem is exhaustively solved, and the fixed points of the renormalization flow are highlighted.

==> figures/M1prim.tikz.tex <==
\begin{tikzpicture}
\draw[black]  (\bitdistance+\bitsize,1)--(\bitdistance+\bitsize,-1);
\draw[black]  (0,1)--(0,-1);
\node[M1] at (\bitsize+\transfoffset,0) {$M_1'$};
\end{tikzpicture}

==> figures/Ucirc.tikz.tex <==
\begin{tikzpicture}
\foreach \t in {0,...,3}{
\draw (\bitsize*\t+\bitdistance*\t,-1)--(\bitsize*\t+\bitdistance*\t,1);
\node[U] at (\bitsize*\t+\bitdistance*\t,0) {$U$};
}
\end{tikzpicture}

==> figures/Uprimeswap.tikz.tex <==
\begin{tikzpicture}
\foreach \t in  {0,1}{
\draw[black]  (\bitdistance*\t+\bitsize*\t,0) -- (\bitdistance*\t+\bitsize*\t, 1.5*\hdist) ;
\node[U]  at (\bitdistance*\t+\bitsize*\t,0.25*\hdist)   {$U'$};
}
\draw[black]  (0,1*\nhdist) -- (\bitdistance+\bitsize,0) ;
\draw[black]  (0,0) -- (\bitdistance+\bitsize,1*\nhdist) ;
\end{tikzpicture}

==> figures/Uswap.tikz-copy.tex <==
\begin{tikzpicture}
\foreach \t in  {0,1}{
\draw[black]  (\bitdistance*\t+\bitsize*\t,0) -- (\bitdistance*\t+\bitsize*\t, 2*\hdist) ;
}
\node[U]  at (0+0,0.25*\hdist)   {$Z'$};
\node[U]  at (\bitdistance*1+\bitsize*1,0.25*\hdist)   {$W$};
\draw[black]  (0,1*\nhdist) -- (\bitdistance+\bitsize,0) ;
\draw[black]  (0,0) -- (\bitdistance+\bitsize,1*\nhdist) ;
\end{tikzpicture}

==> figures/metatikz.tex <==
\usetikzlibrary {arrows.meta}
\usetikzlibrary{%
    decorations.pathreplacing,%
    decorations.pathmorphing,%
    arrows,
    arrows.meta,
    positioning,
    calc,
    shapes,
    shadows,
    shapes.geometric
    }

\definecolor{myblue1}{RGB}{0,157,209}

\tikzset{
  local/.style 2 args={
    rectangle, 
    rounded corners=1pt, 
    minimum height={#1},
    minimum width={#2},
    align=center, 
    line width=1pt,
    draw=white,
    opacity=0.7,
    font=\color{black}\sffamily, 
    fill=myblue1
  },
  local/.default={0.6 cm}{0.6 cm},
  T/.style={
 	rectangle,
 	rounded corners=1pt ,
 	align=center,
 	line width =2pt,
 	draw=black,
 	opacity=0.7,
    font=\color{black}\sffamily, 
    fill=myblue1
  }
 }

==> figures/twocells.tikz.tex <==
\begin{tikzpicture}
\foreach \a in {0,...,1}{
\node[bit] (A\a ) at (\a cm,0) {};
\node at ($(A\a)-(0,1)$) {\a};
}

\end{tikzpicture}

